The Volume of a Local Nodal Domain

Let M either be a closed real analytic Riemannian manifold or a closed smooth Riemannian surface. We estimate from below the volume of a nodal domain component in an arbitrary ball provided that this component enters the ball deeply enough.

==> declarations.tex <==
%-------------------------------------
% declarations file for posvol.tex
%-------------------------------------
\usepackage[centertags]{amsmath}     %what's centertags?
% \usepackage{amsfonts}              loaded automatically with amssymb.
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage{newlfont}               what's this ?
%\usepackage[mathscr]{eucal}         script fonts.
\usepackage{verbatim}                %what's this?
\usepackage[dvips]{graphics}
\usepackage{enumerate}
%\graphicspath{{~/latex/thesis/eps}} doesn't work right.

\renewcommand{\thesection}{\arabic{section}}
\numberwithin{equation}{section}
\newtheorem{prop}[equation]{Proposition}
\newtheorem{lem}[equation]{Lemma}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem{dfn}[equation]{Definition}
\newtheorem{conj}[equation]{Conjecture}
\newtheorem{cor}[equation]{Corollary}
\newtheorem{thm}[equation]{Theorem}
\newtheorem{clm}[equation]{Claim}
\newtheorem{claim}[equation]{Claim}

\newtheorem*{thm1.3p}{Theorem 1.3'}
\newtheorem*{thm1.3pp}{Theorem 1.3''}
\newtheorem*{klem}{Key Lemma}

%\newtheorem{definition_ch}{Definition}[chapter]
%\newtheorem{corollary_ch}[definition_ch]{Corollary}
%\newtheorem{theorem_ch}[definition_ch]{Theorem}

%\newtheorem*{remark}{Remark}
\newcommand{\remark}{\noindent\textbf{Remark.}}
\newcommand{\observation}{\noindent\textbf{Observation.}}
\newcommand{\remarks}{\noindent\textbf{Remarks}}

\newcommand{\me}{\mathrm{e}}
\newcommand{\mi}{\mathrm{i}}
\newcommand{\eps}{\varepsilon}

\newcommand{\tldvphi}{\tilde{\varphi}}
\newcommand{\tldh}{\tilde{h}}
\newcommand{\tld}[1]{{\tilde{#1}}}
\newcommand{\wtld}[1]{{\widetilde{#1}}}
\newcommand{\vphi}{\varphi}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\Rb}{\mathbb{R}}
\newcommand{\Sb}{\mathbb{S}}  % \SS is already occupied
\newcommand{\Tb}{\mathbb{T}}
\newcommand{\ZZ}{\mathbb{Z}}

\newcommand{\Al}{\mathcal{A}}
\newcommand{\Bl}{\mathcal{B}}
\newcommand{\Dl}{\mathcal{D}}
\newcommand{\El}{\mathcal{E}}
\newcommand{\Fl}{\mathcal{F}}
\newcommand{\Hl}{\mathcal{H}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Ml}{\mathcal{M}}
\newcommand{\Nl}{\mathcal{N}}
\newcommand{\Ol}{\mathcal{O}}
\newcommand{\Pl}{\mathcal{P}}
\newcommand{\Ql}{\mathcal{Q}}
\newcommand{\Rl}{\mathcal{R}}
\newcommand{\Sl}{\mathcal{S}}
\newcommand{\Tl}{\mathcal{T}}
\newcommand{\Ul}{\mathcal{U}}
\newcommand{\Vl}{\mathcal{V}}
\newcommand{\Xl}{\mathcal{X}}

\newcommand{\Id}{\mathrm{Id}}
\newcommand{\DIV}{\mathrm{div}}
\newcommand{\PSL}{\mathrm{PSL}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\inrad}{\mathrm{inrad}}
\newcommand{\length}{\mathrm{length}}
\newcommand{\area}{\mathrm{area}}
\newcommand{\Area}{\mathrm{Area}}
\newcommand{\Av}{\mathrm{Av}}
\newcommand{\Vol}{\mathrm{Vol}}
\newcommand{\vol}{\mathrm{vol}}
\newcommand{\Int}{\mathrm{Int}}
\newcommand{\grad}{\mathrm{grad}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\spn}{\mathrm{span}}
\newcommand{\CAP}{\mathrm{cap}}
\newcommand{\Lip}{\mathrm{Lip}}
%\newcommand{\dim}{\mathrm{dim}} already defined.

\newcommand{\genus}{\mathrm{genus}}

\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\bdry}{\partial}
\newcommand{\dif}[1]{{\;d #1}}
\newcommand{\dx}{\;dx}
\newcommand{\dy}{\;dy}
\newcommand{\Op}{\mathrm{Op}}
\newcommand{\Prob}{\mathrm{Prob}}

\newcommand{\Bhf}{\frac{1}{2}B}
\newcommand{\Qhf}{\frac{1}{2}Q}
%\newcommand{\ddr}{\mbox{$\frac{\partial}{\partial r}$}}
%\newcommand{\ddtheta}{\mbox{$\frac{\partial}{\partial \theta}$}}
\newcommand{\dd}[1]{{\textstyle\frac{\partial}{\partial #1}}}
\newcommand{\mdd}[1] {{\frac{\partial}{\partial #1}}}
\newcommand{\tdd}[1] {{\textstyle\partial/\partial #1}}

\newcommand{\hole}{\mathrm{hole}}
\newcommand{\pr}{\mathrm{pr}}

